SYM3D: Learning Symmetric Triplanes for Better 3D-Awareness of GANs

Despite the growing success of 3D-aware GANs, which can be trained on 2D images to generate high-quality 3D assets, they still rely on multi-view images with camera annotations to synthesize sufficient details from all viewing directions. However, the scarce availability of calibrated multi-view image datasets, especially in comparison to single-view images, has limited the potential of 3D GANs. Moreover, while bypassing camera pose annotations with a camera distribution constraint reduces dependence on exact camera parameters, it still struggles to generate a consistent orientation of 3D assets. To this end, we propose SYM3D, a novel 3D-aware GAN designed to leverage the prevalent reflectional symmetry structure found in natural and man-made objects, alongside a proposed view-aware spatial attention mechanism in learning the 3D representation. We evaluate SYM3D on both synthetic (ShapeNet Chairs, Cars, and Airplanes) and real-world datasets (ABO-Chair), demonstrating its superior performance in capturing detailed geometry and texture, even when trained on only single-view images. Finally, we demonstrate the effectiveness of incorporating symmetry regularization in helping reduce artifacts in the modeling of 3D assets in the text-to-3D task. Project is at \url{https://jingyang2017.github.io/sym3d.github.io/}

==> fig/pdf/0_get3d_triplane.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/method/GET3D_Tri.png}
    \caption{Visulization of the geometric tri-plane used in GET3D. The RGB image is a 2D rendering produced by GET3D. The Tri-XY, Tri-YZ, and Tri-XZ images represent the respective planes of the geometry tri-plane that are responsible for generating the RGB image.}
    \label{fig:geo3d_triplane}
\end{figure}

==> fig/pdf/8_orientation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{fig/pdf/orientation.pdf}
    \caption{Orientation learned on different chair dataset}
    \label{fig:oritentation_comp}
\end{figure}

==> tab/tab_att_plane.tex <==
% \begin{figure*}
%  \begin{minipage}[b]{.48\linewidth}
%     \centering
%     \resizebox{0.98\linewidth}{!}{
%     \setlength\tabcolsep{3.5 pt}
%     \begin{tabular}{c|c|c|c}
%     \hline
%     Method    &Added Params &Added Flops  &FID  \\
%     \hline
%     GET3D~\cite{get3d} &0 &0 &55.17\\
%     WinS=4&4616&1.0G&49.83\\
%     WinS=8&6024&1.6G&46.73\\
%     \method{}&294&19.3M&38.23 \\
%     \hline
%     \end{tabular}}
%     \captionof{table}{Comparison using the self-attention module, tested on ShapeNet Chair-S1.}
%     \label{tab:winsa}
%   \end{minipage}
%   \begin{minipage}[b]{.48\linewidth}
%     \centering
%     \resizebox{0.98\linewidth}{!}{
%     \setlength\tabcolsep{3.5 pt}
%     \begin{tabular}{@{}lccccc@{}}
%     \hline
%     \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD ($\downarrow$)} & FID ($\downarrow$) \\ \cmidrule(l){2-6} 
%     & LFD & CD & LFD & CD & 3D \\ \midrule    
%     GET3D~\cite{get3d}&53.73&7.17&4980&5.37&40.66 \\
%     \method{} &\bf{57.85}&\bf{49.07}&\bf{4074}&\bf{1.15}&\bf{32.61}\\
%     \hline
%     \end{tabular}}
%     \captionof{table}{Generality on a more complex category. Experiments are done on ShapeNet Airplane.}
%     \label{tab:plane}
%   \end{minipage}
%   \vspace{-5mm} 
% \end{figure*}

==> tab/tab_car.tex <==
\begin{table}[t]
\centering
% \scriptsize
\vspace{2mm}
\begin{tabular}{@{}clccccc@{}}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD ($\downarrow$)} & FID ($\downarrow$) \\ \cmidrule(l){3-7} 
    & \multicolumn{1}{c}{} & LFD & CD & LFD & CD & 3D \\ \midrule
    \multirow{3}{*}{Car-S1} 
    &OP3D \cite{orthoplanes} &29.24&0.07&2593&13.48&34.23\\
    & GET3D \cite{get3d} &58.30&28.25&1461&1.42&29.69\\
    & \method{}&\bf{63.35}&\bf{36.13}&\bf{1284}&\bf{1.21} &\bf{23.07}\\
    \hline
    \multirow{3}{*}{Car-S2} 
    & OP3D \cite{orthoplanes}&15.69&0.07&3404&18.5&41.49\\
    & GET3D \cite{get3d} &55.96	&19.88	&1731	&1.77&34.60\\
    & \method{} &\bf{65.46}	&\bf{32.86}	&\bf{1708}	&\bf{1.50} & \bf{31.35}\\
    \hline
    \multirow{3}{*}{Car-S3} 
    &OP3D \cite{orthoplanes}&12.43&0.13&3737&20.67&48.19\\
    & GET3D \cite{get3d} &47.79&15.86&1747&1.80&36.39\\
    & \method{} &\bf{50.13}	&\bf{19.88}	&\bf{1709} &\bf{1.69} &\bf{32.81}\\
\hline
\end{tabular}
\caption{Quantitative results on ShapeNet-Car. The best result is shown in \textbf{bold}, and MMD-CD scores are multiplied by $10^3$.}
\label{tab:car}
\vspace{-6mm}
\end{table}

==> tab/tab_chair.tex <==
\begin{table}[t]
\centering
% \scriptsize
% \vspace{2mm}
\begin{tabular}{@{}clccccc@{}}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD ($\downarrow$)} & FID ($\downarrow$) \\ \cmidrule(l){3-7} 
    & \multicolumn{1}{c}{} & LFD & CD & LFD & CD & 3D \\ \midrule
    \multirow{3}{*}{Chair-S1} 
    & OP3D \cite{orthoplanes} &24.4	&0.09	&4183	&34.05&60.82\\
    & GET3D \cite{get3d} &\bf{66.31} & 15.03& 3412 & 14.98 & 55.17 \\
    & \method{} &64.58&\bf{58.53}&\bf{3227}&\bf{4.42}&\bf{38.34} \\
    \hline
    \multirow{3}{*}{Chair-S2} 
    & OP3D \cite{orthoplanes}&32.18&0.18&4764&11.8&74.83\\
    & GET3D \cite{get3d}&\bf{67.29} &15.38 &3754 &14.92 &63.35 \\
    & \method{} &67.02 &\bf{56.32} &\bf{3563} &\bf{4.74} &\bf{51.18}\\
    \hline
% \multirow{2}{*}{Chair-S3} & GET3D &48.98 &31.56 &4497 & 7.70 &99.83\\
%     & \method{} &50.84 &25.02 &4503 &9.28 &86.90 \\
    \multirow{3}{*}{Chair-S3} 
    & OP3D \cite{orthoplanes}&27.76	&0.09	&4853	&15.50&76.40\\
    & GET3D \cite{get3d}&\bf{63.00} &16.00 &3837 & 15.52 &66.51\\
    & \method{} &62.86 &\bf{53.14} &\bf{3661} &\bf{4.94} &\bf{56.59}\\
\hline
\end{tabular}
\caption{Quantitative results on ShapeNet-Chair. The best result is shown in \textbf{bold}, and MMD-CD scores are multiplied by $10^3$.}
\label{tab:chair}
\vspace{-8mm}
\end{table}

==> tab/tab_moto.tex <==
\begin{table}[h]
\centering
\scriptsize
\vspace{2mm}
\begin{tabular}{@{}clccccc@{}}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD ($\downarrow$)} & FID ($\downarrow$) \\ \cmidrule(l){3-7} 
    & \multicolumn{1}{c}{} & LFD & CD & LFD & CD & 3D \\ \midrule
    \multirow{3}{*}{Car-S1} 
    &OP3D\\
    & GET3D &58.3&28.25&1461&1.42&29.69\\
    & \method{}&63.35&36.13&1284&1.21 &23.07\\
    \hline
\hline
\end{tabular}
\caption{Quantitative results on ShapeNet-Motorbike. The best result is shown in \textbf{bold}, and MMD-CD scores are multiplied by $10^3$.}
% \vspace{-10mm}
\label{tab:car}
\end{table}
